MERLOT: Multimodal Neural Script Knowledge Models

As humans, we understand events in the visual world contextually, performing multimodal reasoning across time to make inferences about the past, present, and future. We introduce MERLOT, a model that learns multimodal script knowledge by watching millions of YouTube videos with transcribed speech -- in an entirely label-free, self-supervised manner. By pretraining with a mix of both frame-level (spatial) and video-level (temporal) objectives, our model not only learns to match images to temporally corresponding words, but also to contextualize what is happening globally over time. As a result, MERLOT exhibits strong out-of-the-box representations of temporal commonsense, and achieves state-of-the-art performance on 12 different video QA datasets when finetuned. It also transfers well to the world of static images, allowing models to reason about the dynamic context behind visual scenes. On Visual Commonsense Reasoning, MERLOT answers questions correctly with 80.6% accuracy, outperforming state-of-the-art models of similar size by over 3%, even those that make heavy use of auxiliary supervised data (like object bounding boxes). Ablation analyses demonstrate the complementary importance of: 1) training on videos versus static images; 2) scaling the magnitude and diversity of the pretraining video corpus; and 3) using diverse objectives that encourage full-stack multimodal reasoning, from the recognition to cognition level.

==> figures/attnviz_examples.tex <==
\begin{figure}[h!]
\centering
  \includegraphics[width=\linewidth]{figures/attn_viz/attn_ex0.pdf}
\caption{\modelname~attention patterns, averaged over all layers, show it learns to reason over distant frames and captions. The video is about an e-bike, which is absent from the third frame, the model nevertheless learns to unmask words like `electric' by attending to context further away in time.}
\label{fig:attnvizex}
\end{figure}

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:sec_with_some_limitations}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section~\ref{sec:sec_with_potential_impacts}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We plan to release our model's code either via the supplementary material or on \texttt{github} after acceptance (but prior to publication). }
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We will be including per-dataset discussion of hyperparameters in Appendix.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Many of the datasets we used adopt a leaderboard style format where multiple submissions are not possible, so we were unable to do this. }
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{All the datasets and code used are public and released under licenses managed by the original creators.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{But, we are planning to release our model upon (or before) acceptance.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{We discuss our perspective on this in Section~\ref{sec:sec_with_potential_impacts}.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We didn't do any new crowdworking/human participant experiments for the described work.} 
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tables/t_zeroshot.tex <==
\begin{figure}[t!]
\centering\small
\begin{minipage}{.38\textwidth}
  \centering\scriptsize
    \captionof{table}{Results unscrambling visual stories, on VIST \cite{huang2016visual,agrawal_sort_2016}. The captions are provided in the correct order and models are tasked with sorting the images temporally. \modelname  performs best on all metrics despite being given no training data. }
\begin{tabular}{@{}l@{\hspace{0.25em}}ccc@{}}
& Spearman $(\uparrow)$  & Pairwise acc $(\uparrow)$ & Distance $(\downarrow)$ \\ \hline
CLIP \cite{radford2021learning} & 60.9 & 78.7 & 63.8 \\
UNITER-Base \cite{chen2019uniter} & 54.5 & 75.2 & 74.5 \\
UNITER-Large \cite{chen2019uniter} & 54.3 & 75.1 & 74.5 \\
Ours & \textbf{0.855} & \textbf{89.4} & \textbf{0.396} \\
\end{tabular}
  \label{tab:zero_shot_results}
\end{minipage}%
\hspace{.039\textwidth}\begin{minipage}{.55\textwidth}
  \centering\small
    we can put something else here
%   \captionof{figure}{Example}
\end{minipage}\vspace{-5mm}
\end{figure}
